Cooperative Protocols for Random Access Networks

Cooperative communications have emerged as a significant concept to improve reliability and throughput in wireless systems. On the other hand, WLANs based on random access mechanism have become popular due to ease of deployment and low cost. Since cooperation introduces extra transmissions among the cooperating nodes and therefore increases the number of packet collisions, it is not clear whether there is any benefit from using physical layer cooperation under random access. In this paper, we develop new low complexity cooperative protocols for random access that outperform the conventional non cooperative scheme for a large range of signal-to-noise ratios.

==> Makefile <==
PROJECT=allerton08
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps

default: no_bib

clean:
	rm -f $(TMPFILES);
clean_pdf:
	rm -f $(PROJECT).pdf;


final: clean clean_pdf
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	bibtex $(PROJECT);
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -Ppdf -t letter -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dEmbedAllFonts=true\
 -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

no_bib: 
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

literatur:
	cp ~/Desktop/work/freia/references/trunk/Literatur.bib ./;
	cp ~/Desktop/work/freia/references/trunk/confs-jrnls.bib ./;


==> acknowledgement.tex <==
\section*{Acknowledgment}


==> results.tex <==
\section{Numeric Results}
\subsection{Overall Energy Constraint}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{../images/throughputsNoCoop}
\caption{Throughputs for direct link with perfect TDMA (dashed line), direct
link, 2-Hop and simplified decode-forward with cooperation on the MAC layer
(blue, red and green line respectively) and simplified decode-forward without
cooperation on the MAC layer (line in cyan). As can be seen, the lack of
cooperation on the MAC layer leads to a degradation by a factor in high SNR.}
\label{fig:throughputs}
\end{figure}
and the max-min throughput becomes
\begin{align}
\ssdf=\max_{\gammaall,\timeall,\tau}\min\left\{\degnocoop\csdf^{\nnear},
\degnocoop\csdf^{\nfar}\right\}.
\end{align}
Note this degradation factor differs from the degeneration factor for no
cooperation on the MAC layer by the term $\ptrans\timef$.
The max-min throughput becomes
\begin{align}
\ssdf=\max_{\gammaall,\timeall,\tau}\min\left\{\degcoop\csdf^{\nnear},
\degcoop\csdf^{\nfar}\right\}.
\end{align}
As can be seen in Figure \ref{fig:throughputs}, lack of cooperation on the MAC
layer leads to a throughput degradation by a factor in high SNR.
\subsection{Per-Node Power Constraint}
\myemph{
give practical arguments for choosen parameter space
}
